Experimental investigation of the limitations of polarisation optics for future gravitational wave detectors based on the polarisation Sagnac speedmeter

The polarisation Sagnac speedmeter interferometer has the potential to replace the Michelson interferometer as the instrumental basis for future generations of ground-based gravitational wave detectors. The quantum noise benefit of this speedmeter is dependent on high-quality polarisation optics, the polarisation beam-splitter (PBS) and quarter-waveplate (QWP) optics that are key to this detector configuration and careful consideration of the effect of birefringence in the arm cavities of the interferometer. A PBS with an extinction ratio of better than 4000 in transmission and 700 in reflection for a $41^{\circ}$ angle of incidence was characterised along with a QWP of birefringence of $\frac{\lambda}{4} + \frac{\lambda}{324}$. The cavity mirror optics of a 10m prototype polarisation Sagnac speedmeter were measured to have birefringence in the range $1\times10^{-3}$ to $2\times10^{-5}$ radians. This level of birefringence, along with the QWP imperfections, can be canceled out by careful adjustment of the QWP angle, to the extent that the extinction ratio of the PBS is the leading limitation for the polarisation Sagnac speedmeter in terms of polarisation effects.

==> Bib.tex <==
%%  [1] 
@article{aLIGO,
  author = {J. Aasi {\it et al} (The LIGO Scientific Collaboration)},
   title = {Advanced {LIGO}},
   journal = {Class. Quantum Grav.},
   volume = {32},
   year = {2015},
   pages = {074001},
}   

%%  [2] 
@article{aVirgo,
  author = {F. Acernese {\it et al} (Virgo Collaboration)},
   title = {{Advanced {V}irgo: {A} {S}econd-Generation Interferometric Gravitational Wave Detector}},
  journal = {Class.Quantum Grav.},
  volume = {32},
  number = {2},
  year = {2015},
  pages = {024001},
}

%%  [3] 
@article{O1O2cat1,
      author = {B. P. Abbott {\it et al} (LIGO Scientific Collaboration and Virgo Collaboration)},
      title = {{GWTC-1: A Gravitational-Wave Transient Catalog of Compact Binary Mergers Observed by LIGO and Virgo during the First and Second Observing Runs}},
  collaboration = {LIGO Scientific Collaboration and Virgo Collaboration},
  journal = {Phys. Rev. X},
  volume = {9},
  issue = {3},
  pages = {031040},
  numpages = {49},
  year = {2019},
  month = {Sep},
}

%%  [4] 
@article{GWTC2,
author = {R. Abbott  {\it et al} (LIGO Scientific Collaboration and Virgo Collaboration)},
year = {2020},
month = {10},
pages = {},
title = {{GWTC}-2: Compact Binary Coalescences Observed by {LIGO and Virgo} During the First Half of the Third Observing Run}
}

%%  [5] 
@article{InterferometryLivRev,
  author = {{Freise}, A. and {Strain}, K.},
  title = {{Interferometer Techniques for Gravitational-Wave Detection}}, 
  year = {2010},
  journal = {Living Review in Relativity},
  volume = {13},
  number = {1},
}

%%  [6] 
@article{Buikema20,
  title = {Sensitivity and performance of the {Advanced LIGO} detectors in the third observing run},
  author = {A. Buikema {\it et al}},
  journal = {Phys. Rev. D},
  volume = {102},
  issue = {6},
  pages = {062003},
  numpages = {27},
  year = {2020},
  month = {Sep},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevD.102.062003},
  url = {https://link.aps.org/doi/10.1103/PhysRevD.102.062003}
}

%%  [7]
@article{Acernese19,
  title = {Increasing the Astrophysical Reach of the {Advanced Virgo} Detector via the Application of Squeezed Vacuum States of Light},
  author = {F. Acernese {\it et al}},
  collaboration = {Virgo Collaboration},
  journal = {Phys. Rev. Lett.},
  volume = {123},
  issue = {23},
  pages = {231108},
  numpages = {10},
  year = {2019},
  month = {Dec},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.123.231108},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.123.231108}
}


%%  [8] 
@Article{Bode20,
AUTHOR = {N. Bode {\it et al}},
TITLE = {Advanced {LIGO} Laser Systems for {O3} and Future Observation Runs},
JOURNAL = {Galaxies},
VOLUME = {8},
YEAR = {2020},
NUMBER = {4},
ARTICLE-NUMBER = {84},
URL = {https://www.mdpi.com/2075-4434/8/4/84},
ISSN = {2075-4434},
DOI = {10.3390/galaxies8040084}
}

%%  [9] 
@article{Tse19,
  title = {Quantum-Enhanced {Advanced LIGO} Detectors in the Era of Gravitational-Wave Astronomy},
  author = {M. Tse {\it et al}},
  journal = {Phys. Rev. Lett.},
  volume = {123},
  issue = {23},
  pages = {231107},
  numpages = {8},
  year = {2019},
  month = {Dec},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.123.231107},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.123.231107}
}

%%  [10] 
@Article{Mehmet20,
AUTHOR = {{Mehmet}, M. and {Vahlbruch}, H.},
TITLE = {The Squeezed Light Source for the {Advanced Virgo} Detector in the Observation Run {O3}},
JOURNAL = {Galaxies},
VOLUME = {8},
YEAR = {2020},
NUMBER = {4},
ARTICLE-NUMBER = {79},
URL = {https://www.mdpi.com/2075-4434/8/4/79},
ISSN = {2075-4434},
DOI = {10.3390/galaxies8040079}
}

%%  [11] 
@article{Corbitt04,
  author = {{Corbitt}, T. and {Mavalvala}, N.},
  title = {{Quantum Noise in Gravitational Wave Interferometers}},
  journal = {Journal of Optics B},
  year = {2004},
  volume = {6},
  number = {8},
}

%%  [12] 
@article{FirstSpeedmeter,
  author = {{Braginsky}, V. and {Khalili}, F.},
  title = {{Gravitational Wave Antenna with {QND} Speed Meter}},
  year = {1990},
  journal = {Phy. Lett. A},
  volume = {147},
  pages = {251},
}
%%  [13] 
@article{QMTLivRev,
  author = {{Danilishin}, S. and {Khalili}, F.},
  title = {{Quantum Measurement Theory in Gravitational Wave Detectors}},
  journal = {Living Reviews in Relativity},
  year = {2012},
  volume = {15},
  number = {5},
}
%%  [14] 
@article{ET10,
	doi = {10.1088/0264-9381/27/19/194002},
	year = {2010},
	month = {Sep},
	publisher = {{IOP} Publishing},
	volume = {27},
	number = {19},
	pages = {194002},
	author = {M. Punturo {\it et al}},
	title = {{The Einstein Telescope: a third-generation gravitational wave observatory}},
	journal = {Classical and Quantum Gravity},
}


%%  [15] 
@article{DanilishinPolSM,
  author = {{Danilishin}, S.},
  title = {{Sensitivity Limitations in Optical Speed Meter Topology of Gravitational-Wave Antennas}},
  journal = {Phy. Rev. D},
  year = {2004},
  volume ={69},
  pages = {102003},
}

%%  [16] 
@article{ChenRing,
  author = {{Chen}, Y.},
  title = {{Sagnac Interferometer as a Speed-Meter-Type, Quantum-Nondemolition Gravitational-Wave Detector}},
  journal = {Phy. Rev. D},
  year = {2003},
  volume = {67},
  pages = {122004},
}

%%  [17] 

@article{PurdueChenSlosh,
  author = {{Purdue}, P. and {Chen}, Y.},
  title = {{Practical Speed Meter Designs for Quantum Nondemolition Gravitational-Wave Interferometers}},
  journal = {Phy. Rev. D},
  year = {2002},
  volume = {66},
  pages = {122004},
}

%%  [18] 
@article{Huttner,
  author = {S. Huttner {\it et al}},
  title = {{Candidates for a Possible Third-Generation Gravitational Wave Detector: Comparison of ring-Sagnac and sloshing-Sagnac speedmeter interferometers}},
  journal = {Class. Quantum Grav.},
  year = {2016},
  volume = {34},
  number = {2},
}

%%  [19] 
@article{DanilishinPolCirc,
  author = {{Danilishin}, S. and {Knyazev}, E. and {Voronchev}, N. and {Khalili}, F. and {Gr{\"a}f}, C. and {Steinlechner}, S. and {Hennig}, J. and {Hild}, S.},
  title = {{A New Type of Quantum Speed Meter Interferometer Measuring Speed to Search for Intermediate Mass Black Holes.}},
  journal = {Light Science and Applications},
  year = {2018},
  volume = {7},
  number={11},
}

%%  [20] 
@article{EPR,
title = {{Speedmeter Scheme for Gravitational-Wave Detectors Based on EPR Quantum Entanglement}},
author = {{Knyazev}, E. and {Danilishin},S. and {Hild},S. and {Khalili},F.},
journal = {Physics Letters A},
volume = {382},
number = {33},
pages = {2219 - 2225},
year = {2018},
}

%%  [21] 
@article{AsymmerticSSM,
  author = {{Danilishin}, S. and {Gräf}, C. and {Leavey}, S. and {Hennig}, J. and {Houston}, E. and {Pascucci}, D. and {Steinlechner}, S. and {Wright}, J. and {Hild}, S.},
  title = {{Quantum Noise of Non-Ideal {S}agnac Speed Meter Interferometer with Asymmetries}},
  journal = {New Journal of Physics},
  volume = {17},
  year = {2015},
}
   
   
%%  [23] 
@article{Calcite,
author = {{Skeldon},K.D. and {Clubley},D.A. and {Newton}, G.P. and {Thieux}, S. and {Von Gradowski}, M. and {Barr}, B.W.},
year = {2001},
month = {Mar},
pages = {695-702},
title = {{Measurements of an Ultra-Low Loss Polarizer for $\lambda =$1064 nm Using a High Finesse Optical Cavity}},
volume = {48},
journal = {Journal of Modern Optics},
}


%%  [25] 
@book{PolShurcliff,
  author = {{Shurcliff}, W.},
  title = {{Polarized Light Production and Use}},
  year = {1962},
  publisher = {Harvard University Press},
}

%%  [26] 
@article{BirefringenceMoriwaki,
  author = {{Moriwaki}, S. and {Sakaida}, H. and {Yuzawa}, T. and {Mio}, N.},
  title = {{Measurement of the Residual Birefringence of Interferential Mirrors Using {Fabry-Perot} Cavity}},
  year = {1997},
 journal = {Appl. Phys. B},
  volume = {65},
  number = {},
  pages = {347-350},
} 

%%  [27] 
@article{BirefringenceBrandi,
author = {{Brandi}, F. and {Della Valle}, F. and {De Riva}, A.M. and {Micossi}, P. and {Perrone}, F. and {Rizzo}, C. and {Ruoso}, G. and {Zavattini}, G.},
year = {1997},
month = {Sept},
pages = {351-355},
title = {{Measurement of the Phase Anisotropy of Very High Reflectivity Interferential Mirrors}},
volume = {65},
journal = {Applied Physics B},
doi = {10.1007/s003400050283},
}

%%  [28] 
@article{BirefringenceJacob,
author = {{Jacob},D. and {Vallet},M. and {Bretenaker},F. and {Le Floch},A. and {Oger},M.},
journal = {Opt. Lett.},
keywords = {Anisotropy; Birefringence; Crosstalk; Optical coatings; Polarization; Prisms},
number = {7},
pages = {671--673},
publisher = {OSA},
title = {{Supermirror Phase Anisotropy Measurement}},
volume = {20},
month = {Apr},
year = {1995},
url = {http://ol.osa.org/abstract.cfm?URI=ol-20-7-671},
doi = {10.1364/OL.20.000671},
abstract = {The high sensitivity of the eigenstates of a large-finesse passive Fabry -- Perot cavity is used to measure the residual anisotropy of supermirrors at strictly normal incidence. An experimental demonstration leads to the measurement of phase retardances of the order of 10{\textminus}6 rad.},
}

%%  [29] 
@article{BirefringenceReview,
  author = {{Bielsa}, F. and {Dupays}, A. and {Fouche}, M. and {Battesti}, R. and {Robilliard}, C. and {Rizzo}, C.},
  title = {{Birefringence of Interferential Mirrors at Normal Incidence (Experimental and Computational study)}},
  year = {2009},
  journal = {Appl. Phys. B},
  volume = {97},
  number = {2},
  pages = {457-463},
} 


%%  [30] 
@article{Cole16,
  author = {G. Cole {\it et al}},
  title = {{High-Performance Near- and Mid-Infrared Crystalline Coatings}},
  year = {2016},
  journal = {Optica},
  volume = {3},
  number = {},
  pages = {647656},
}

%%  [31] 
@article{Winkler,
title = {{Birefringence-induced losses in interferometers}},
author = {{Winkler}, W. and {Rüdiger}, A. and {Schilling}, R. and {Strain}, K.A. and {Danzmann}, K.},
year =  {1994},
journal = {Optics Communications},
volume = 	{112},
number = {5-6},
pages =	{245-252},
}

%%  [34] 
@misc{ETDesign,
  author = {M. Punturo {\it et al}},
  title = {Einstein gravitational wave Telescope ({ET}) conceptual design study},
  year = {2011},
  howpublished = {http://www.et-gw.eu/index.php/relevant-et-documents},
}




%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%	      Misc        		%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%
@Phdthesis{SpencerPhD,
  author  = {{Spencer},A.P.},
  title  = {{Advanced techniques in laser interferometry for current and future gravitational wave detectors}},
  school	= {{University of Glasgow}},
  type  = {{PhD Thesis}},
  year  = {2020},
}

@misc{Layertech,
  title = {{Layertec}},
  howpublished = {https://www.layertec.de/en/},
}

@misc{UOptic,
  title = {{Union Optic}},
  howpublished = {https://www.u-optic.com/},
}

@article{CDS,
author = {{Bork}, R. and {Abbott}, R. and {Barker}, D. and {Heefner}, J.},
year = {2001},
month = {Jan},
pages = {19-23},
journal = {Proc. ICALEPCS},
title = {{An Overview of the {LIGO} Control and Data Acquisition Systems}},
}

@misc{Matlab,
  title = {{MATLAB is a registered trademark of The Math Works, Inc.}},
  howpublished = {https://uk.mathworks.com/products/matlab.html},
}

@misc{TowerOptic,
  title = {{Tower Optic}},
  howpublished = {https://www.toweroptical.com/4-zero-order-waveplates/},
}

